Near log-convexity of measured heat in (discrete) time and consequences

Let $u,v \in \mathbb{R}^\Omega_+$ be positive unit vectors and $S\in\mathbb{R}^{\Omega\times\Omega}_+$ be a symmetric substochastic matrix. For an integer $t\ge 0$, let $m_t = \smash{\left\langle v,S^tu\right\rangle}$, which we view as the heat measured by $v$ after an initial heat configuration $u$ is let to diffuse for $t$ time steps according to $S$. Since $S$ is entropy improving, one may intuit that $m_t$ should not change too rapidly over time. We give the following formalizations of this intuition. We prove that $m_{t+2} \ge m_t^{1+2/t}\!,$ an inequality studied earlier by Blakley and Dixon (also Erd\H{o}s and Simonovits) for $u=v$ and shown true under the restriction $m_t\ge e^{-4t}$. Moreover we prove that for any $\epsilon>0$, a stronger inequality $m_{t+2} \ge t^{1-\epsilon}\cdot \smash{m_t^{1+2/t}}$ holds unless $m_{t+2}m_{t-2}\ge \delta m_t^2$ for some $\delta$ that depends on $\epsilon$ only. Phrased differently, $\forall \epsilon> 0, \exists \delta> 0$ such that $\forall S,u,v$ \begin{equation*} \frac{m_{t+2}}{m_{t}^{1+2/t}}\ge \min\left\{t^{1-\epsilon}, \delta\frac{m_t^{1-2/t}}{m_{t-2}}\right\}, \quad \forall t \ge 2, \end{equation*} which can be viewed as a truncated log-convexity statement. Using this inequality, we answer two related open questions in complexity theory: Any property tester for $k$-linearity requires $\Omega(k\log k)$ queries and the randomized communication complexity of the $k$-Hamming distance problem is $\Omega(k\log k)$. Further we show that any randomized parity decision tree computing $k$-Hamming weight has size $\exp\left(\Omega(k\log k)\right)$.

==> definitions/proceedings.tex <==

\usepackage[utf8]{inputenc}
\usepackage{hyperref}
\usepackage{amsmath, amsthm, amssymb}
\usepackage{accents}
\usepackage{microtype}
\usepackage[usenames]{xcolor}
\usepackage{nicefrac}
\usepackage{bbm}
\definecolor{Blue}{RGB}{5, 55, 77}
\definecolor{Red}{RGB}{20,50,10}
\usepackage{pgfplots}
\usepackage {tikz}
\usetikzlibrary {positioning}
\usepackage{float}
\usepackage{aliascnt}
\usepackage{multirow}
\hypersetup{
    colorlinks,
    citecolor=Red,
    filecolor=Blue,
    linkcolor=Blue,
    urlcolor=Blue,
    breaklinks=false,
}
\usepackage{enumerate}
\usepackage{mathtools}


==> definitions/theoremlike.tex <==
\numberwithin{equation}{section}
\makeatletter
\let\oldtheequation\theequation
\renewcommand\tagform@[1]{\maketag@@@{\ignorespaces#1\unskip\@@italiccorr}}
\renewcommand\theequation{(\oldtheequation)}
\makeatother
\renewcommand{\equationautorefname}{Eq.}



\DeclareMathSymbol{\widehatsym}{\mathord}{largesymbols}{"62}
\newcommand\lowerwidehatsym{%
  \text{\smash{\raisebox{-1.3ex}{%
    $\widehatsym$}}}}
\newcommand\fixwidehat[1]{%
  \mathchoice
    {\accentset{\displaystyle\lowerwidehatsym}{#1}}
    {\accentset{\textstyle\lowerwidehatsym}{#1}}
    {\accentset{\scriptstyle\lowerwidehatsym}{#1}}
    {\accentset{\scriptscriptstyle\lowerwidehatsym}{#1}}
}

\newcommand{\indicator}{\mathbf 1}
\newcommand{\indicate}[1]{\mathbbm{1}_{#1}}

\newcommand{\Ham}{\mathrm{Ham}}
\newcommand{\Disj}{\mathrm{Disj}}
\newcommand{\Ghd}{\mathrm{GHD}}

\makeatletter
\newcommand*{\defeq}{\mathrel{\rlap{%
                     \raisebox{0.3ex}{$\cdot$}}%
                     \raisebox{-0.3ex}{$\cdot$}}%
                     =}
\makeatother

\newcommand{\conv}{\mathrm{conv}}
\newcommand{\sfrac}[2]{\nicefrac{#1}{#2}}
\newcommand{\onehalf}{\nicefrac{1}{2}}
\newcommand{\stirling}[2]{{#1 \brack #2}}
\newcommand{\cmid}{\,:\,}
\newcommand{\trans}[1]{\widehat{#1}}
\newcommand{\translow}[1]{\fixwidehat{#1}}
\newcommand{\parenth}[1]{\left(#1\right)}
\newcommand{\nparen}[1]{\left(#1\right)}
\newcommand{\sparen}[1]{\left[#1\right]}
\newcommand{\cparen}[1]{\left\{#1\right\}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\eps}{\epsilon}
\newcommand{\lebd}{\,\mathrm{d}}
\newcommand{\diff}[1]{\mathrm{d} #1}
\newcommand{\idiff}[1]{\,\mathrm{d} #1}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}


\newtheorem{theorem}{Theorem}[section]

%Conjecture
  \newaliascnt{conjecture}{theorem}
  \newtheorem{conjecture}[conjecture]{Conjecture}
  \aliascntresetthe{conjecture}
  \def\conjectureautorefname{Conjecture}

%Corollary
  \newaliascnt{corollary}{theorem}
  \newtheorem{corollary}[corollary]{Corollary}
  \aliascntresetthe{corollary}

\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{fact}{Fact}[section]
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

\def\claimautorefname{Claim}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\lemmaautorefname{Lemma}
\def\propositionautorefname{Proposition}
\def\factautorefname{Fact}

